Quantifying Grover speed-ups beyond asymptotic analysis

Run-times of quantum algorithms are often studied via an asymptotic, worst-case analysis. Whilst useful, such a comparison can often fall short: it is not uncommon for algorithms with a large worst-case run-time to end up performing well on instances of practical interest. To remedy this it is necessary to resort to run-time analyses of a more empirical nature, which for sufficiently small input sizes can be performed on a quantum device or a simulation thereof. For larger input sizes, alternative approaches are required. In this paper we consider an approach that combines classical emulation with detailed complexity bounds that include all constants. We simulate quantum algorithms by running classical versions of the sub-routines, whilst simultaneously collecting information about what the run-time of the quantum routine would have been if it were run instead. To do this accurately and efficiently for very large input sizes, we describe an estimation procedure and prove that it obtains upper bounds on the true expected complexity of the quantum algorithms. We apply our method to some simple quantum speedups of classical heuristic algorithms for solving the well-studied MAX-$k$-SAT optimization problem. This requires rigorous bounds (including all constants) on the expected- and worst-case complexities of two important quantum sub-routines: Grover search with an unknown number of marked items, and quantum maximum-finding. These improve upon existing results and might be of broader interest. Amongst other results, we found that the classical heuristic algorithms we studied did not offer significant quantum speedups despite the existence of a theoretical per-step speedup. This suggests that an empirical analysis such as the one we implement in this paper already yields insights beyond those that can be seen by an asymptotic analysis alone.

==> overview.tex <==
\section{Overview of papers}
\subsection{Quantifying Grover speed-ups beyond asymptotic analysis}
\paragraph{Main story:}
we propose a method to numerically analyse the performance of quantum algorithms that rely on Grover-like subroutines to attain a (sub)-quadratic asymptotic speed-up in an oracle setting. 
\paragraph{Structure:}
\begin{enumerate}
    \item Introduction
    \item Preliminaries
    \begin{itemize}
        \item Grover (with an unknown number of marked items)
    \end{itemize}
    \item Methodology (results)
    Lemmas + theorems for:
    \begin{itemize}
        \item Query complexity bounds when the fraction is known
        \item Query complexity bounds by sampling
    \end{itemize}
    \item A case study: MAX-$k$-SAT hill climber
    \begin{itemize}
        \item Asymptotic behaviour
        \item Numerics (scaling + real data-sets)
    \end{itemize}
    \item Conclusion
\end{enumerate}
\paragraph{Other ideas/future work:}
\begin{itemize}
    \item Sampling without replacement
\end{itemize}

\newpage

\subsection{Quantum algorithms for community detection}
\paragraph{Main story:}
 we propose quantum algorithms, based on the Louvain algorithm, for the community detection problem. By studying both the asymptotic complexity and estimates for query counts on actual data sets by utilizing the method of paper 1, we find that A) and B) etc.
 \paragraph{Structure:}
\begin{enumerate}
    \item Introduction
    \item Preliminaries
        \begin{itemize}
        \item Notation
        \item Community detection
        \item The Louvain algorithm
    \end{itemize}
    \item Complexity of the Louvain algorithm
    \begin{itemize}
        \item Complexity measures
          \item Data structure
    \end{itemize}
    \item Quantum algorithms
    (Theorems for with asymptotic scaling for all proposed quantum algorithms).
    \begin{itemize}
        \item Quantum Louvain
        \item Simple quantum Louvain
        \item Trading a square root for a log factor for sparse graphs
        \item Quantum with variable time amplitude amplification
        \item Edge-search Louvain
        \item Node-neighbouring community Louvain
    \end{itemize}
    \item Numerical results
    \begin{itemize}
        \item Comparison absolute query counts for Louvain and quantum algorithms.
        \item Artificial and real-life networks.
    \end{itemize}
    \item Conclusion
\end{enumerate}
\paragraph{Other ideas/future work:}
\begin{itemize}
    \item 
\end{itemize}


